First Measurements of the 4-Point Correlation Function of Magnetohydrodynamic Turbulence as a Novel Probe of the Interstellar Medium

In the Interstellar Medium (ISM), gas and dust evolve under magnetohydrodynamic (MHD) turbulence. This produces dense, non-linear structures that then seed star formation. Observationally and theoretically, turbulence is quantified by summary statistics such as the 2-Point Correlation Function (2PCF) or its Fourier-space analog the power spectrum. These cannot capture the non-Gaussian correlations coming from turbulence's highly non-linear nature. We here for the first time apply the 4-Point Correlation Function (4PCF) to turbulence, measuring it on a large suite of MHD simulations that mirror, as well as currently possible, the conditions expected in the ISM. The 4PCF captures the dependence of correlations between quadruplets of density points on the geometry of the tetrahedron they form. Using a novel functionality added to the \textsc{sarabande} code specifically for this work, we isolate the purely non-Gaussian piece of the 4PCF. We then explore simulations with a range of pressures, $P$, and magnetic fields, $B$ (but without self-gravity); these are quantified by different sonic $(M_{\rm S})$ and Alfv\'enic $(M_{\rm A})$ Mach numbers. We show that the 4PCF has rich behavior that can in future be used as a diagnostic of ISM conditions. We also show that a large-scale coherent magnetic field leads to parity-odd modes of the 4PCF, a clean test of magnetic field coherence with observational ramifications. All our measurements of the 4PCF (10 $M_{\rm S}, M_{\rm A}$ combinations, 9 time-slices for each, 34 4PCF modes for each) are made public for the community to explore.

==> sections/01_introduction.tex <==
The gas of the interstellar medium (ISM) plays a crucial role in star formation and connecting stellar and galactic scales. Gas provides the material needed to form stars, while turbulence influences the dynamics of star formation processes. They influence the gravitational collapse of material, allow for the growth of protostellar disks, help stars reach main sequence by increasing their mass to the point that nuclear fusion can begin, and halt the star formation process as they interact with radiation (\cite{Williams_2005_dustgas}). These processes ultimately replenish the ISM with matter and energy, connecting stars and larger galactic scales, further emphasizing the importance of understanding the role of gas fully.

The interstellar medium is greatly turbulent and magnetized, complicating studies further (\cite{Mckee_2007_starform}, \cite{Elmegreen_2004_ISM}). Turbulence refers to the irregular motion of gas and dust, and it is characterized by a power-law energy spectrum, suggesting it to be an organized phenomena filled with eddies. Turbulence affects nearly all regions of the ISM and is the primary factor driving the diffusion of matter and dissipation of kinetic energy (\cite{Falceta-Goncalves_2014_turbulence}). Many believe that understanding turbulence is the most essential step to understanding star formation as a whole. The magnetized ISM interacts with charged particles and the magnetic fields of other objects. Like turbulence, magnetic fields are also predicted to play a larger role in star formation than we currently understand through their impact on the dynamics of the medium. It affects the behavior of charged particles and opposes forces of gravity, reducing fragmentation of massive dense cores and working against the contraction of these cores (\cite{Motte_2021_highmass}. Therefore, a greater understanding of star formation processes and the ISM as a whole will require studies accounting for both these factors.

Magnetohydrodynamic (MHD) simulations offer a way to investigate these turbulent density structures in the ISM. The CATS turbulence simulations are one of the MHD simulations that can reproduce these important characteristics of the ISM. However, these simulations could be made more accurate in the future with the help of measurements of non-Gaussian information on real data.  In recent years, the field has turned to exploring higher-order statistics such as 3-Point Correlation Functions (3PCF) and its Fourier space analog, the bispectrum. \cite{Slepian_2015_3pcfon^2} introduced an algorithm that has greatly reduced the 3PCF computational time and expense, which has been applied to large scale structure (\cite{Slepian_2017_largescale3pcf}) and on turbulence in the interstellar medium with the Fourier-Transform-based version  (\cite{Portillo_2018_3pcfISM}). These current state of the art algorithms measure the 3PCF by using spherical harmonics to create an isotropic orthonormal basis (\cite{Slepian_2015_3pcfon^2} ). On a grid, angular basis functions are created, which are then radially binned to create kernels and convolved with the original gridded data to obtain the expansion coefficients at each point simultaneously. The combination of these coefficients gives us the 3PCF as this orthonormal basis (\cite{Sunseri_2022_SARABANDE}). They are able to gather more information about non-Gaussian interactions in the density fields than the 2-Point Correlation Function or its Fourier analog the Power Spectrum multiple orders of magnitude faster. 

Despite the success of the 3PCF, there are limitations and disadvantages to using this method because since the 3PCF has contributions from the 2PCF, but these contributions are not easily separable, the 3PCF is not favorable for studying only non-Gaussian information. \cite{Philcox_2022_ENCORE}, \cite{Cahn_2021_ParityViolation}, \cite{Philcox_2021_disconnected}, and \cite{Hou_2022_oddparity} explore the use of the 4-Point Correlation Function as an alternative. The greatest strength of the 4PCF over the 3PCF is its sensitivity to Non-Gaussianity.  When employing the 3PCF, we are unable to remove the non-Gaussian parts of the data collected, but with the 4PCF it is possible. Additionally, the 4PCF is favorable to measuring the turbulent interstellar medium because it is sensitive to parity violation (\cite{Hou_2022_oddparity}, \cite{Philcox_2022_Probing}) and more sensitive to the non-linear equations of magnetic fields, potentially making it more sensitive to magnetic field directions. 

Here, we present the first ever usage of the 4-Point Correlation Function on MHD simulations of the Interstellar Medium. The recent release of the \texttt{python}  package \textsc{sarabande} (\cite{Sunseri_2022_SARABANDE}) allows for the measurement of the 4PCF in $\mathcal{O}(N_{\mathrm{gm}} \log N_{\mathrm{gm}})
$ time using Fast Fourier Transforms (FFTs), with $N_{\mathrm{gm}}$ the number of grid points used for the FFT. \textsc{sarabande} requires analysis on regular gridded data sets, for which the MHD simulations of density fields in the ISM satisfy. With our access to this code, we are uniquely positioned to make the first measurements of non-Gaussian information from the gathered data in order to measure the connected 4PCF.

% \begin{itemize}
%     \item Introduce why topic important (ISM/turbulence stuff)
%     \item Limits to simulations
%     \item Ppl have started using higher order statistics: 3PCF
%     \item problems faced by 3PCF
%     \item Introduce 4PCF, why so much better
%     \item first ppl to ever do this, have access to code, only ppl able to remove non Gaussian bits
%     \item paper is structured as follows...
% \end{itemize}
% \begin{itemize}
%     \item sell it, why should anyone care
%     \item why is 4PCF better than 3PCF for star formation: sensitive to parity, more sensitive to non Gaussianity, more sensitive to mag fields non-linear equations (might be sensitive to mag field directions)
    % \item Characterize gas in ISM and understand how stars form, problem b/c power spectrum only and 3PCF only one paper on it
    % \item PCF sensitive to nonGaussian in way 3PCF isnt
    % \item never measured the 4PCF, only ppl who can measure the connected (removes Gaussian, non-important info)
    % \item series of papers to develop NPCF recently, SARABANDE has been released fro 4PCF with FFT (talk abt nlogN scaling) using gridded data sets (perfect to this)
    
    % The 3PCF is a natural tool for turbulence studies as it encodes information about non-linear interactions that is absent in the 2-Point Correlation Function (2PCF), the configuration-space analog of the power spectrum.
% 3pcf not good because cant remove the non gaussian bits, 4pcf can

This paper is structured as follows: Section \ref{sec:Methods} describes the underlying mathematics behind the \textsc{sarabande} code, the MHD simulations we use, and the supercomputers used to run these simulations. Section \ref{sec:Analysis} outlines the scaling methodology, the connected 4PCF, and angular and dependence of the function. Section \ref{sec:Results} presents our measurements and explains patterns seen in the data. Section \ref{sec:Conclusion} concludes our findings and presents future applications of the work.

% The interstellar medium (ISM) is all of the matter and radiation existing between star systems, in the form of gas, dust, and cosmic rays. The three-phase model (Field, Goldsmith \& Habing (1969) and McKee \& Ostriker(1977)) describes the ISM in temperature-dependent phases: (1) a cold (T<300 K) dense phase consisting of clouds of hydrogen, (2) a warm (T $\simeq 10^4$ K) intercloud phase of neutral and ionized gas, and (3) very hot (T $\simeq 10^6$ K) gas shock heated by supernovae. 

% Magnetic fields and turbulence play the largest role in creating pressure in the ISM. 

% The turbulence of the ISM means it plays a crucial role in star formation and connecting stellar and galactic scales. Stars are born inside large molecular clouds, the densest regions of the ISM. Throughout their lifetimes, stars interact with the ISM by building up molecular clouds and replenishing the ISM with matter and energy, through planetary nebalue, stellar winds, and supernovae.

% The 4PCF has been known to be sensitive to parity-odd signals (\cite{Hou_2022_oddparity})

==> sections/02_methods.tex <==
\james{I think it's always good to have a little overview of the breakdown of this section. I hate seeing 2 section headers right next to each other.}
\subsection{SARABANDE}
The code we run on these MHD simulations is the \texttt{python}  package \textsc{sarabande} developed in \cite{Sunseri_2022_SARABANDE}. \textsc{sarabande} uses the 4 Point Correlation Function, fully discussed and derived in \cite{Philcox_2022_ENCORE} and \cite{Cahn_2020_isotropicNP}. The full 4PCF uses 4 points in the estimator, creating a tetrahedral geometry with the three vectors The full 4PCF in its most basic form is written as 
\begin{equation}
\label{eq:full_zeta_angle}
    \zeta = \langle \delta(\vec{x})\delta(\vec{x}+\vec{r}_1)\delta(\vec{x}+\vec{r}_2)\delta(\vec{x}+\vec{r}_3) \rangle_\mathcal{R}.
\end{equation}
The left-hand side of the equation has arguments left unstated purposely due to the different ways to parameterize the full 4PCF. Here the lengths of the tetrahedron are defined by $r_1$, $r_2$, and $r_3$, while the angles between them are $\vec{r}_1$,  $\vec{r}_2$, and $\vec{r}_3$. \cite{Cahn_2020_isotropicNP} explores the angular dependence of the 4PCF through isotropic basis functions. The sum of radial coefficients $\zeta_{\Lambda}$ times these isotropic basis functions $\mathcal{P}_{\Lambda}$ represent the full 4PCF alternatively: 
\begin{equation}
\label{4pcf_basis}
    \zeta = \sum_{\Lambda} \hat{\zeta}_{\Lambda}^{R} \mathcal{P}_{\Lambda}(\hat{R}).
\end{equation}
We define $\Lambda = {\ell_1, \ell_2, \ell_3}$ as the set of angular momenta used to describe the quadruplet angles used for the full 4PCF. In equation \ref{4pcf_basis} the isotropic orthonormal basis function is defined as
\begin{equation}
    \mathcal{P}_{\Lambda}(\hat{R}) = \sum_{M} C^{\Lambda}_{M} Y_{\ell_1 m_1}(\hat{r}_1) Y_{\ell_2 m_2}(\hat{r}_2) Y_{\ell_3 m_3}(\hat{r}_3),
\end{equation}
% The lengths of said tetrahedron are defined by $r_1$, $r_2$, and $r_3$, while the angles between them are $\vec(r_1), \vec(r_2), \vec(r_3)$. 
and $C^{\Lambda}_{M}$ is given by the Wigner 3-$j$ symbol with an additional phase:
\begin{equation}
    C^{\Lambda}_{M} = (-1)^{\ell_1 + \ell_2 + \ell_3} \begin{pmatrix}
\ell_1 & \ell_2 & \ell_3\\
m_1 & m_2 & m_3
\end{pmatrix}.
\end{equation}
 In the equations above, we define $M \equiv(m_1,m_2,m_3)$, $\hat{R} \equiv (\hat{r}_1,\hat{r}_2,\hat{r}_3)$, and $R \equiv(r_1, r_2, r_3)$. The full 4PCF must be computed using the radial coefficients shown in equation \ref{4pcf_basis}. This can be done in terms of binned convolution coefficients $a_{\ell m}^{\rm b}(\vec{x})$, defined by
 \begin{align}
\label{eqn:almconv}
    a^{\rm b}_{\ell m}(\vec{x}) = \int d^3\vec{r}\; Y_{\ell m}^*(\hat{r})\Phi^{\rm b}(r)\delta(\vec{x} + \vec{r}).
\end{align}
The binning function $\Phi^{\rm b}$ used above is described by
\begin{align}
    \Phi^{\rm b}(r) = \frac{\Theta^{\rm b}(r)}{V_{\rm b}}.
\label{eq:bin_volume_unity}
\end{align}
The result is the radial coefficients about each point $\vec{x}$ defined as
\begin{multline}
    \hat{\zeta}_{\ell_1 \ell_2 \ell_3}^{\; \rm b_1 \rm b_2 \rm b_3}(\vec{x}) = \delta(\vec{x})\sum_{M} \mathcal{E}(\Lambda) \; C^{\Lambda}_{M} \\ \times \; a_{\ell_1 m_1}^{\rm b_1}(\vec{x}) \; a_{\ell_2 m_2}^{\rm b_2}(\vec{x}) \; a_{\ell_3 m_3}^{\rm b_3}(\vec{x}).
\label{eqn:mu}
\end{multline}
$\mathcal{E}(\Lambda)$ is +1 for even parity, occurring when $l_1+l_2+l_3$ is an even number, and -1 for odd parity, occurring when this value is an odd number.

To ensure dimensionless results and consistent weighting, \textsc{sarabande} normalizes each radial bin by its volume, which accounts for variations in the number of grid cells within each bin. The bin volume is calculated as:
\begin{equation}
    V_{\text{bin}} = \left(\frac{L}{N_{\text{mesh}}}\right)^3 N_{\text{cells in bin}},
\end{equation}
where $L$ is the box size, $N_{\text{mesh}}$ is the grid resolution per dimension, and $N_{\text{cells in bin}}$ is the number of grid cells in the bin. This normalization prevents artifacts arising from varying bin sizes and ensures the 4PCF accurately reflects physical correlations.

The scales analyzed using \textsc{sarabande} range from the smallest measurable grid resolution to half the box size. Limiting the maximum scale to $L/2$ avoids redundant information due to periodic boundary conditions while covering the inertial range of turbulence, where critical non-Gaussian features emerge. These scale choices optimize the analysis for capturing the physical processes driving MHD turbulence.
 
\subsection{Simulations of MHD Turbulence}
% \graphicspath{{figures/figures/sim_slices.png}}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/figures/sim_slices.png}
    \caption{Sample density field slices of the selected MHD sets used in this work, shown using a logarithmic color map. This demonstrates the correlation between higher sonic and Mach-Alfv\'enic numbers and small scale filaments of high density. Slower movement allows time for the small-scale power in the fluid to diminish and smooth out existing filaments.}
    \label{fig:sim_slices}
\end{figure*}

The MHD simulations we used to obtain the density profiles for sub- and supersonic turbulent gas with varying magnetic field strengths were isothermal and non-self-gravitating. To exclude outside factors, we employ the ideal MHD equations solved in other works (\cite{Portillo_2018_3pcfISM}),
\begin{equation}
    \frac{\partial \rho}{\partial t} + \nabla \cdot (\rho \vec{\varv}) = 0,
 \label{eq:MHD_1st}
\end{equation}
\begin{equation}
    \frac{\partial (\rho \vec{\varv})}{\partial t} + \nabla \cdot [\rho \vec{\varv} \vec{\varv} + (p + \frac{B^2}{8\pi})\vec{I} - \frac{1}{4\pi} \vec{B}\vec{B}] = \vec{f},
 \label{eq:MHD_2nd}
\end{equation}
\begin{equation}
    \frac{\partial \vec{B}}{\partial t} - \nabla \times (\vec{v} \ \times \vec{B}) = 0 \label{eq:MHD_3rd}
\end{equation}
 where $\rho$ is the density, $\vec{B}$, is the magnetic field, \textit{p} is the gas pressure, $\vec{I}$ is the identity matrix, and $\vec{B}\vec{B}$ is the magnetic stress matrix. Equation \ref{eq:MHD_1st} is the continuity equation which represents conservation of mass demonstrates how the change in mass over time plus the divergence of mass flow rate over the unit area must be zero. Equation \ref{eq:MHD_2nd} represents conservation of momentum, stating that the change in momentum over time plus the divergence of momentum flex, plus the gradient of pressure and magnetic force must equal the external forces acting on the fluid. Equation \ref{eq:MHD_3rd} represents conservation of magnetic flux by demonstrating that the rate of change of the magnetic field over time minus the curl of the velocity-induced magnetic field must be zero. We assume zero-divergence condition, periodic boundary conditions, and an isothermal equation of state. We assume a wave number of $k = 2.5$, where k is expressed in terms of the number of cells in the simulation grid. The wave number is 1/2.5 the box size and is driving a large-scale solenoidal for the source term $\vec{f}$. The simulations runs used are available as part of the Catalog for Astrophysical Turbulence Simulations (\cite{Burkhart2020}, \cite{Burkart_Lazarian_2016}, \cite{Cho_2003_MHD}).

Our simulations explore varying parameters of sonic Mach numbers and Alfv\'enic Mach numbers, with $v$ as the velocity, $c_{s}$ as sound speed, and $v_A$ as the Alfv\'en speed. Our simulations run with $M_S$ $\simeq$ 0.7, 1.2, and 7.0, and $M_A$ $\simeq$ 0.7 and 2.0.

Any desired physical scale can be assigned for the box size, since the simulations are non-self-gravitating. We use $\approx$ when stating the sonic and Alfv\'enic Mach numbers because they are averages which fluctuate slightly over time.

The resulting density fields from these simulations are shown in Figure \ref{fig:sim_slices}, where we present sample slices using a logarithmic color map. These slices illustrate how varying Mach numbers influence the density structure. Higher sonic and Alfvénic Mach numbers are associated with small-scale filaments of high density, while lower Mach numbers show smoother structures with less prominent filamentation. The slower motion of the gas in subsonic regimes allows time for the small-scale power in the fluid to diminish, smoothing out existing filaments, as evidenced by the smoother density field. These visualizations help contextualize the turbulent structures present in the simulations and set the stage for our subsequent analysis of the 4PCF.

\subsection{Architecture}
% We ran the 4PCF calculations on the University of Florida's supercomputer, HiPerGator, and Princeton University's supercomputer, Della.

% \james{Moving from your abstract: We performed these computations on the HiPerGator (University of Florida) and Della (Princeton University) supercomputers with an estimated 45,000+ CPU Hours.}

\james{
To measure the connected 4PCF on all 50+ simulations, we used high-performance computing clusters at both Princeton University (Della) and University of Florida (HiperGator). The Della cluster at Princeton University is a heterogeneous cluster supporting several different computer architectures. For our analysis, we exclusively used nodes with 2.4 GHz Intel Broadwell Central Processing Units (CPUs). Each node contains 28 CPUs with a total shared memory of 128 GBs. The max instruction set for cores is AVX2. 
\\
The \textsc{sarabande} package uses an \textsc{OpenMP} parallelization paradigm to unravel nested \texttt{for} loops necessary for the combining binned convolution coefficients $a_{\ell \rm m}^{\rm b}$ into the radial 4PCF coefficients $\zeta^{\rm b_1 b_2 b_3}_{\rm \ell_1 \ell_2 \ell_3}$. Using an entire node (28 Broadwell CPUs) on the Della Cluster, \textsc{sarabande} measured the connected 4PCF with an $\ell_{\rm max} = 3$ at a 
radial resolution of 20 bins for a single 256$^3$ data cube in $\sim 24$ Wall Hours.
}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/figures/sarabande_process_b3=10.png}
    \caption{This depicts the process by which the 4PCF was calculated throughout this paper. The updated version of the \textsc{sarabande} python package utilized in this work is able to separate the connected and disconnected pieces of the data, allowing us to isolate the non-Gaussian information. This work can be recreated by collecting the full data and subtracting off the disconnected piece, which holds the 2PCF and Gaussian information already studied in other works (\protect\cite{Portillo_2018_3pcfISM}), to leave behind only the connected piece containing 4PCF data.}
    \label{fig:sarabande_process_b3=10}
\end{figure*}

==> sections/03_analysis.tex <==
\subsection{Normalization and Scaling}
Before applying \textsc{sarabande} to compute the 4PCF, the density fields from our MHD simulations undergo a preliminary processing step to standardize the data and emphasize non-Gaussian structures. The density fields of turbulent media are often log-normal, meaning the logarithm of the density fluctuations follows a Gaussian distribution (\cite{vazquez_1994_hierarchical}, \cite{federrath_2008_density}, 
\cite{burkhart_2011)_stattools}). To enable meaningful statistical analysis, we scale the density field as follows:
\begin{equation}
    \delta = \frac{\log \rho - \langle \log \rho \rangle}{\sigma(\log \rho)},
 \label{eq:log_scale}
\end{equation}
where $\rho$ is the density field, $\langle \log \rho \rangle$ is the mean logarithm of the density, and $\sigma(\log \rho)$ is its standard deviation (\cite{Portillo_2018_3pcfISM}. This transformation forces the density fluctuation field for each simulation cube to have zero mean and unit variance. We then take the 4PCF of this density fluctuation field. This normalization allows for consistent comparisons across simulations with varying Mach and Alfv\'enic numbers. It enables \textsc{sarabande} to isolate higher-order statistical features for detection and analysis.

\subsection{The Connected 4PCF}
While the full 4PCF is sensitive to non-Gaussian information, it is difficult to isolate the most meaningful information that can't be studied with a simple power spectrum or 2PCF. This is because, unlike the 2PCF and 3PCF, the 4PCF consists of two constituent parts: a connected piece and a disconnected piece. 
\begin{equation}
    \hat{\zeta} = \hat{\zeta}^{\rm (connected)} + \hat{\zeta}^{(\rm disconnected)}
\end{equation}
The disconnected piece is degenerate, consisting of products of 2PCFs which are not sensitive to non-Gaussian information. In this work we isolate the connected piece of the 4PCF as done in \cite{Philcox_2021_disconnected} to extract only the most important non-Gaussian information the 4PCF has to offer. To isolate the connected piece we first refer back to Eq. \ref{eq:full_zeta_angle} and recognize that the averaging over realizations in the product of four density fluctuation fields can be decomposed as
\begin{multline}
\label{eq:disconnected_1}
    \langle \delta(\vec{x})\delta(\vec{x}+\vec{r}_1)\delta(\vec{x}+\vec{r}_2)\delta(\vec{x}+\vec{r}_3) \rangle_\mathcal{R} = \\ \langle \delta(\vec{x})\delta(\vec{x}+\vec{r}_1)\delta(\vec{x}+\vec{r}_2)\delta(\vec{x}+\vec{r}_3) \rangle_{\mathcal{R}}^{(c)} \\ + \underbrace{[\langle \delta(\vec{x})\delta(\vec{x}+\vec{r}_1) \rangle_\mathcal{R} \langle \delta(\vec{x}+\vec{r}_2)\delta(\vec{x}+\vec{r}_3) \rangle_\mathcal{R} + \rm 2 \; Perms.]}_{\rm Disconnected \; Piece}.
\end{multline}
Recognizing that the average over realizations and rotations of the product of two density fluctuation fields is the 2PCF, we can then rewrite as
\begin{equation}
    \zeta = \zeta^{\rm (c)} + \underbrace{[\xi(\vec{r}_1) \xi(\vec{r}_2 - \vec{r}_3) + \rm 2 \; Perms.]}_{\rm Disconnected \; Piece}.
\end{equation}
Following the derivation in \cite{Philcox_2021_disconnected} we can write the resulting disconnected 4PCF as 
\begin{equation}
    \hat{\zeta}_{\ell_1 \ell_2 \ell_3}^{\; \rm b_1 \rm b_2 \rm b_3 (disc)}(\vec{x}) = C^{\Lambda}_{M} \left( \hat{\xi}_{\ell_1 m_1}^{\; \rm b_1} \hat{\xi}_{\ell_2 m_2 \ell_3 m_3}^{\; \rm b_2 b_3} + \rm 2 \; Perms. \right).
\end{equation}
With this disconnected piece we can now subtract it off from the full 4PCF and isolate the desired connected pieace. Using an updated version of \textsc{sarabande} in this work, we isolate the connected piece through this process, depicted visually in Figure \ref{fig:sarabande_process_b3=10}.

\subsection{Angular and Parity Dependence}
To fully capture the angular information in the 4PCF, we use Legendre polynomials and isotropic basis functions to expand the angular dependence between tetrahedral sides. This expansion introduces multipole moments, indexed by $l_1$, $l_2$, $l_3$, which represent the angular structure of the 4PCF. Even-parity components, where $l_1$ + $l_2$ + $l_3$ is even, dominate the signal. This reflects the inherent symmetries we find in turbulence. The odd-parity components, where $l_1$ + $l_2$ + $l_3$ is odd, are weaker but offer insight into asymmetries in the density field from magnetic fields, anisotropic turbulence driving, and other interesting factors. For the sake of computational efficiency, the expansion is halted at $l_{\text{max}}$ = 5.

% \graphicspath{{figures/figures/1d_start/}}

\begin{figure} % Inline positioning
    \centering
    \begin{subfigure}{0.50\textwidth} % First image, less than half the width
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{Figures/figures/1d_plots/1dplot_ell0.png}
        \label{fig:1d_ell=0}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.50\textwidth} % Second image, less than half the width
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{Figures/figures/1d_plots/1dplot_ell1.png}
        \label{fig:1d_ell=1}
    \end{subfigure}
    \caption{The 1-dimensional 4PCF for $l_1$, $l_2$, $l_3$ = 0 and $l_1$, $l_2$, $l_3$ = 1.}
    \label{fig:1d_start}
\end{figure}

% \graphicspath{{figures/figures/1d_end/}}

\begin{figure} % Inline positioning
    \centering
    \begin{subfigure}{0.50\textwidth} % First image, less than half the width
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{Figures/figures/1d_plots/1dplot_ell2.png}
        \label{fig:1d_ell=2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.50\textwidth} % Second image, less than half the width
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{Figures/figures/1d_plots/1dplot_ell3.png}
        \label{fig:1d_ell=3}
    \end{subfigure}
    \caption{The 1-dimensional 4PCF for $l_1$, $l_2$, $l_3$ = 2 and $l_1$, $l_2$, $l_3$ = 3.}
    \label{fig:1d_end}
\end{figure}


==> sections/04_results.tex <==
In this work, we present the first ever measurements of the connected 4PCF on simulations of MHD turbulence in the ISM, as seen in Figures \ref{fig:1.b_start}, \ref{fig:1.b_end}, \ref{fig:2.b_start}, \ref{fig:2.b_start}, \ref{fig:3.b_start}, \ref{fig:3.b_end}, \ref{fig:4.b_start}, \ref{fig:4.b_end}, \ref{fig:5.b_start}, \ref{fig:5.b_end}, \ref{fig:6.b_start}, \ref{fig:6.b_end}, \ref{fig:7.b_start}, \ref{fig:7.b_end}, \ref{fig:8.b_start}, \ref{fig:8.b_end}, \ref{fig:9.b_start}, and \ref{fig:9.b_end}. These visuals illustrate significant excess and deficit correlation in certain regions. Dark red regions correspond to excess tetrahedra relative to a random distribution, while dark blue regions indicate a deficit. The darkest regions, where values approach +8 and -8 on the color bar, correspond to the strongest detections, where non-Gaussian correlations intrinsic to the density field are most likely to be represented. Regions of lighter coloring, closer to 0 on the the color bar, reflect minimal to no detection of correlation and are more likely consistent with noise.

Our initial interpretations of this data show that we have clearly detected the Connected 4PCF, a direct probe of non-Gaussian information in magnetohydrodynamic simulations. Our application of \textsc{sarabande} analyzed only the non-Gaussian pieces of information by removing 2PCF data, what we refer to as the “disconnected” piece of the data (Figure \ref{fig:sarabande_process_b3=10}). Therefore, any produced results from this study would indicate detectability of the 4PCF, disproving a null hypothesis and effectively granting us measurements not possible to gain from 2PCF or 3PCF studies. 

Visually, it is clear that even-parity components, particularly those represented by $l_1$, $l_2$, $l_3$= 2, dominate the signal. This is consistent with theoretical predictions, since even-parity configurations align with the isotropic symmetries of turbulence. Within the even-parity parameters, $l_1$, $l_2$, $l_3$= 0 appears faint because it represents the 2PCF data that, as explained previously, has been removed during our calculations. The higher-order information displayed by $l_1$, $l_2$, $l_3$= 2 is much stronger because it contains the 4PCF or “connected” part instead. Odd-parity components, such as $l_1$, $l_2$, $l_3$= (3, 2, 2), are fainter but remain detectable. This suggests that subtle asymmetries are present, which could be linked to a variety of factors such as anisotropic driving forces or magnetic field effects. 

The findings also offer insight into the sensitivity of the connected 4PCF to sonic Mach numbers and Alfv\'enic Mach numbers. Supersonic and sub-Alfv\'enic numbers exhibit the strongest non-Gaussian signals. This is likely due to enhanced density contrasts and magnetic field-driven anisotropies. In contrast, subsonic and super-Alfv\'enic conditions display weaker correlations, which is consistent with the reduction of non-linear interactions in these regions.
% \graphicspath{{figures/figures/fullpowerlaw.png}}
% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/figures/fullpowerlaw.png}
%     \caption{The power spectrum of the simulation density fields. The blue line represents the power spectrum averaged over all time slices, while the orange line represents the respective power law fit. The slope of each power law fit is included. The shaded region to the left of the red dotted line, situated at 1.2 x $10^-1$, represent the values outside the inertial range, where the power law no longer follows the power spectrum.}
%     \label{fig:fullpowerlaw}
% \end{figure*}
Exploration of these findings in later papers could attempt to further explain the role the ISM plays in star formation. There is a possibility for \textsc{sarabande} and the methodology employed in this work to be utilized on small regions of the intergalactic medium, likely only within parameters in which turbulence could dominate over the gravitational pull of galaxies. 

\subsection{Implications}
These findings demonstrate the powerful ability of the 4PCF as a probe for non-Gaussian features in turbulent mediums. By isolating the connected component, this methodology is able to efficiently gain access to information that was previously impossible with lower-order statistics such the 2PCF or 3PCF. This work lays a foundation for using the 4PCF to study the ISM, providing insights into the role of turbulence and magnetic fields in star formation. 

Another promising direction for future work from these results is exploring parity-odd components to better understand the role they play in turbulence. Figures \ref{fig:1d_start} and \ref{fig:1d_end} condense the 4PCF coefficients, for a set of $l$ combinations, into 1-dimension to allow further comparison of even and odd parity. This can be replicated for other $l$ combinations in future studies to better understand these results. Parity-odd could be investigated through the data displayed in Figure \ref{fig:fullpowerlaw}. This figure depicts the power spectrum and power law fit of the connected 4PCF data, which when tested for covariance can determine an above null detection by eliminating the possibility of noise detection in the data and confirming that the results could not have been modeled with 2PCFs or power spectra.

We plan to extend this framework to observational datasets to validate its applicability beyond simulations. By applying \textsc{sarabande} to CO emission maps, we will measure the projected 4PCF of real data (\cite{kim_2017_TIGRESS}). "Projected" refers to integrating out the line of sight so that the 3D density field becomes 2D, which is crucial for extracting meaningful 4PCF signals from real density fields (\cite{Sunseri_2022_SARABANDE}). From this we can conduct the first ever 4PCF study of the ISM with feedback, and establish a foundation for exploring how feedback shapes galaxy evolution and star formation.


==> sections/05_conclusions.tex <==
This study repesents the first-ever application of the 4-Point Correlation Function (4PCF) to magnetohydrodynamic turbulence simulations of the interstellar medium (ISM). Our detection of non-Gaussian correlations in the density field demonstrate the significant value of the 4PCF in probing high-order features of turbulence that cannot be captured by traditional 2PCF or 3PCF analyses. By isolating the connected component, with the use of the python package \textsc{sarabande}, we were able to efficiently analyze over 50 simulations with varying sonic Mach and Alfv\'enic Mach parameters. This work revealed new patterns and correlations that are crucial to developing a more comprehensive understanding of turbulence and star formation in the ISM.

In agreement with theoretical predictions, we found that even-parity components dominated the signal, suggesting isotropic symmetries of turbulence play a significant role in their dynamics. The detection of odd-parity components in any regard is significant in opening avenues for the role of subtle asymmetries and anisotropic forces driving turbulence.

The computational framework developed in this work lays the groundwork for future investigations into the complex relationship between turbulence, magnetic fields, and star formation. It establishes the 4PCF as a tool to study complex astrophysical systems as we plan to expand the range of simulations analyzed and integrate observational data to further enhance our understanding of turbulence in shaping the ISM.

% \clearpage
% \graphicspath{{figures/figures/1.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
%     \centering
    
%     \begin{subfigure}{\textwidth} 
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/1.b1=0.png}
%         \label{fig:1.b1=0}
%     \end{subfigure}

%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/1.b1=5.png} 
%         \label{fig:1.b1=5}
%     \end{subfigure}
   
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$ = 0, 1, 2, and 3. The first image shows these $l$ combinations when $b_1$ = 0, and the second image shows when $b_1$ = 5.}
%     \label{fig:1.b_start}
% \end{figure}

% \clearpage
% \graphicspath{{figures/figures/1.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/1.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:1.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/1.b1=15.png} % Image name without extra folder path

%         \label{fig:1.b1=15}
%     \end{subfigure}
%     \centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$ = 0, 1, 2, and 3. The first image shows these $l$ combinations when $b_1$ = 10, and the second image shows when $b_1$ = 15.}
% 	\label{fig:1.b_end}
% \end{figure}

% \clearpage
% \graphicspath{{figures/figures/2.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/2.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:1.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/2.b1=5.png} % Image name without extra folder path

%         \label{fig:1.b1=5}
%     \end{subfigure}
%     \centering
%     \caption{ This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (0,1,1), $l_1$, $l_2$, $l_3$= (0,2,2), $l_1$, $l_2$, $l_3$= (0,3,3), and $l_1$, $l_2$, $l_3$= (1,0,1). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
% 	\label{fig:2.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/2.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/2.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:1.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/2.b1=15.png} % Image name without extra folder path

%         \label{fig:1.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{ This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (0,1,1), $l_1$, $l_2$, $l_3$= (0,2,2), $l_1$, $l_2$, $l_3$= (0,3,3), and $l_1$, $l_2$, $l_3$= (1,0,1). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
% 	\label{fig:2.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/3.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/3.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:3.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/3.b1=5.png} % Image name without extra folder path

%         \label{fig:3.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (1,1,0), $l_1$, $l_2$, $l_3$= (1,1,2), $l_1$, $l_2$, $l_3$= (1,2,1), and $l_1$, $l_2$, $l_3$= (1,2,2). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
% 	\label{fig:3.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/3.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/3.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:3.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/3.b1=15.png} % Image name without extra folder path

%         \label{fig:3.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (1,1,0), $l_1$, $l_2$, $l_3$= (1,1,2), $l_1$, $l_2$, $l_3$= (1,2,1), and $l_1$, $l_2$, $l_3$= (1,2,2). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
% 	\label{fig:3.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/4.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/4.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:4.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/4.b1=5.png} % Image name without extra folder path

%         \label{fig:4.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (1,2,3), $l_1$, $l_2$, $l_3$= (1,3,2), $l_1$, $l_2$, $l_3$= (1,3,3), and $l_1$, $l_2$, $l_3$= (2,0,2). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
% 	\label{fig:4.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/4.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/4.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:4.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/4.b1=15.png} % Image name without extra folder path

%         \label{fig:4.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (1,2,3), $l_1$, $l_2$, $l_3$= (1,3,2), $l_1$, $l_2$, $l_3$= (1,3,3), and $l_1$, $l_2$, $l_3$= (2,0,2). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
% 	\label{fig:4.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/5.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/5.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:5.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/5.b1=5.png} % Image name without extra folder path

%         \label{fig:5.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (2,2,3), $l_1$, $l_2$, $l_3$= (2,1,2), $l_1$, $l_2$, $l_3$= (2,1,3), and $l_1$, $l_2$, $l_3$= (2,2,0). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
% 	\label{fig:5.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/5.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/5.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:5.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/5.b1=15.png} % Image name without extra folder path

%         \label{fig:5.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (2,2,3), $l_1$, $l_2$, $l_3$= (2,1,2), $l_1$, $l_2$, $l_3$= (2,1,3), and $l_1$, $l_2$, $l_3$= (2,2,0). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
%     \label{fig:5.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/6.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/6.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:6.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/6.b1=5.png} % Image name without extra folder path

%         \label{fig:6.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (2,2,1), $l_1$, $l_2$, $l_3$= (2,2,3), $l_1$, $l_2$, $l_3$= (2,3,1), and $l_1$, $l_2$, $l_3$= (2,3,2). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
%     \label{fig:6.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/6.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/6.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:6.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/6.b1=15.png} % Image name without extra folder path

%         \label{fig:6.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (2,2,1), $l_1$, $l_2$, $l_3$= (2,2,3), $l_1$, $l_2$, $l_3$= (2,3,1), and $l_1$, $l_2$, $l_3$= (2,3,2). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
%     \label{fig:6.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/7.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/7.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:7.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/7.b1=5.png} % Image name without extra folder path

%         \label{fig:7.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (2,3,3), $l_1$, $l_2$, $l_3$= (3,0,3), $l_1$, $l_2$, $l_3$= (3,1,2), and $l_1$, $l_2$, $l_3$= (3,1,3). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
%     \label{fig:7.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/7.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/7.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:7.b10=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/7.b1=15.png} % Image name without extra folder path

%         \label{fig:7.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (2,3,3), $l_1$, $l_2$, $l_3$= (3,0,3), $l_1$, $l_2$, $l_3$= (3,1,2), and $l_1$, $l_2$, $l_3$= (3,1,3). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
%     \label{fig:7.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/8.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/8.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:8.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/8.b1=5.png} % Image name without extra folder path

%         \label{fig:8.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (3,2,1), $l_1$, $l_2$, $l_3$= (3,2,2), $l_1$, $l_2$, $l_3$= (3,2,3), and $l_1$, $l_2$, $l_3$= (3,3,0). The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
%     \label{fig:8.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/8.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/8.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:8.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/8.b1=15.png} % Image name without extra folder path

%         \label{fig:8.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (3,2,1), $l_1$, $l_2$, $l_3$= (3,2,2), $l_1$, $l_2$, $l_3$= (3,2,3), and $l_1$, $l_2$, $l_3$= (3,3,0). The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
%     \label{fig:8.b_end}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/9.b_start/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/9.b1=0.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:9.b1=0}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/9.b1=5.png} % Image name without extra folder path

%         \label{fig:9.b1=5}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (3,3,0), $l_1$, $l_2$, $l_3$= (3,3,1), $l_1$, $l_2$, $l_3$= (3,3,2), and $l_1$, $l_2$, $l_3$= (3,3,3). The combination $l_1$, $l_2$, $l_3$= (3,3,3) is repeated solely for the purpose including four combinations in the all plots. The first image shows these $l$ combinations when $b_1$=0 and the second image shows when $b_1$=5.}
%     \label{fig:9.b_start}
% \end{figure}
% \clearpage
% \graphicspath{{figures/figures/9.b_end/}}

% \begin{figure} % Ensure the figure is placed on its own page
% 	\centering
% 	\begin{subfigure}{\textwidth} 
%         \centering
% 		\includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/9.b1=10.png}
%         % Image name without extra folder path due to \graphicspath
% 		\label{fig:9.b1=10}
% 	\end{subfigure}
	
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth, height=0.45\textheight]{Figures/figures/condensed4pcfplt/9.b1=15.png} % Image name without extra folder path

%         \label{fig:9.b1=15}
%     \end{subfigure}
% 	\centering
%     \caption{This is the connected 4PCF for $l_1$, $l_2$, $l_3$= (3,3,0), $l_1$, $l_2$, $l_3$= (3,3,1), $l_1$, $l_2$, $l_3$= (3,3,2), and $l_1$, $l_2$, $l_3$= (3,3,3). The combination $l_1$, $l_2$, $l_3$= (3,3,3) is repeated solely for the purpose including four combinations in the all plots. The first image shows these $l$ combinations when $b_1$=10 and the second image shows when $b_1$=15.}
%     \label{fig:9.b_end}
% \end{figure}
% \clearpage
